Multi-fidelity Bayesian Optimisation with Continuous Approximations

Bandit methods for black-box optimisation, such as Bayesian optimisation, are used in a variety of applications including hyper-parameter tuning and experiment design. Recently, \emph{multi-fidelity} methods have garnered considerable attention since function evaluations have become increasingly expensive in such applications. Multi-fidelity methods use cheap approximations to the function of interest to speed up the overall optimisation process. However, most multi-fidelity methods assume only a finite number of approximations. In many practical applications however, a continuous spectrum of approximations might be available. For instance, when tuning an expensive neural network, one might choose to approximate the cross validation performance using less data $N$ and/or few training iterations $T$. Here, the approximations are best viewed as arising out of a continuous two dimensional space $(N,T)$. In this work, we develop a Bayesian optimisation method, BOCA, for this setting. We characterise its theoretical properties and show that it achieves better regret than than strategies which ignore the approximations. BOCA outperforms several other baselines in synthetic and real experiments.

==> _ <==
\section{Preliminaries}
\label{sec:prelims}

\subsection{A Review of Gaussian processes and \gpucb}
\label{sec:prelims}

\textbf{Gaussian processes:}
A GP over a space $\Xcal$ is a random process describing functions from $\Xcal$ to $\RR$.
It is characterised by a mean function $\mu:\Xcal\rightarrow\RR$ and
a covariance kernel $\kernel:\Xcal^2\rightarrow\RR$.
If $\func\sim\GP(\mu,\kernel)$, then $f(x)$ is distributed normally
$\Ncal(\mu(x), \kernel(x,x))$ for all $x\in\Xcal$.
Suppose we are given $n$ observations from this GP, $\Dcal_n=\{(x_i, y_i)\}_{i=1}^n$ where
$x_i\in\Xcal$, $y_i = \func(x_i) + \epsilon_i \in\RR$ and $\epsilon_i\sim\Ncal(0,\eta^2)$.
Then the posterior process $\func|\Dcal_n$ is also a GP with some mean $\mu_n$ and
covariance $\kernel_n$.
We refer readers unfamiliar with GPs to chapter 2 of~\citet{rasmussen06gps} for
the formulae for $\mu_n,\kernel_n$ and other properties of GPs.

\insertFigBWSample
\textbf{Radial kernels:}
Radial kernels are commonly used in the prior covariance of GPs;
% The squared exponential (SE) kernel and \matern{} kernels, which are popularly used in
% practice, are radial kernels.
some examples are the squared exponential (SE) and \matern{} kernels~\citep{rasmussen06gps}.
When using a radial kernel,
the prior covariance can be written as $\kernel(x,x') = \kernelscale\phi(\|x-x'\|)$ and
depends only on the distance between $x$ and $x'$.
Here, the scale parameter $\kernelscale$ 
captures the magnitude $\func$ could deviate from $\mu$.
The radial kernel, $\phi:\RR_{+}\rightarrow\RR_+$, is a decreasing function with
$\|\phi\|_\infty = \phi(0) = 1$.
In what follows, we will use the SE kernel in a running example to convey the
intuitions in our methods. 
For the SE kernel, $\phi(r) = \radialh(r) = \exp(-r^2/(2h^2))$, where $h$ is
the bandwidth parameter.
It is well known that when $h$ is large, the sample functions drawn from the GP tend to
be smoother as illustrated in Fig.~\ref{fig:gpBWSample}.
We will reference this observation frequently in the text.


\textbf{\gpucb:}
The Gaussian Process Upper Confidence Bound (\gpucb) algorithm
of~\citet{srinivas10gpbandits}  is a method for bandit optimisation,
which, like many other \bayos methods, models $\func$ as a sample from a Gaussian process.
At time $t$, the next point $\xt$ for evaluating $\func$ is chosen via the following
procedure.
First, we construct an upper confidence bound
$\utilt(x) = \mutmo(x) + \betath \sigmatmo(x)$ for the GP. 
$\mutmo$ is the posterior mean of the GP conditioned on the previous $t-1$ evaluations
and $\sigmatmo$ is the posterior standard deviation.
The $\mutmo$ term encourages an \emph{exploitative} strategy -- in that we want to query
regions where we already believe  $\func$ is high -- and $\sigmatmo$ encourages
an \emph{exploratory} strategy -- in that we want to query where we are uncertain
about $\func$ so that we do not miss regions which have not been queried yet.
$\betath$ controls the trade-off between exploration and exploitation.


\subsection{Problem Set Up}
\label{sec:prelims}

In stochastic bandit optimisation, our goal is to maximise a function
$\func:\Xcal\rightarrow \RR$, over a domain $\Xcal$.
When we evaluate $\func$ at $x\in\Xcal$ we observe $y=\func(x) + \epsilon$ where
$\EE[\epsilon] = 0$.
Let $\xopt \in \argmax_{x\in\Xcal}\func(x)$ be a maximiser of $\func$ and
$\funcopt = \func(\xopt)$ be the maximum value.
% $\func$ is accessible only via noisy point evaluations and has no gradient information.
An algorithm for bandit optimisation is a sequence of points $\{\xt\}_{t\geq0}$, where
at time $t$, the algorithm chooses to evaluate $\func$ at $\xt$ based on previous queries
and observations $\{(\xtt{i},\ytt{i})\}_{i=1}^{t-1}$.
After $n$ queries to $\func$,
its goal is to achieve small \emph{simple regret} $\Sn$, as defined below.
\begin{align*}
\Sn = \min_{t=1,\dots,n} \funcopt - \func(\xt).
\numberthis
\label{eqn:SnDefn}
\end{align*}
In this work, we will assume that $\func$ itself is a slice of a function $\gunc$ that lies
in a larger space.
Precisely, we will assume the existence of a fidelity space $\Zcal$ and a function 
$\gunc:\Zcal\times\Xcal \rightarrow \RR$.
The function $\func$ which we wish to maximise is related to $\gunc$ via
$\func(\cdot) = \gunc(\zhf, \cdot)$, where $\zhf\in\Zcal$.
For instance, in the hyper-parameter tuning example discussed in Section~\ref{sec:intro},
$\Zcal = [1,\Nmax]\times[1,\Tmax]$ and $\zhf = [\Nmax, \Tmax]$.
Our goal is to find the maximiser $\xopt = \argmax_x \func(x) = \argmax_x \gunc(\zhf, x)$.
We have illustrated this set up in Figure~\ref{fig:fidelSpace}.
\insertFigFidelSpace

The multi-fidelity framework is attractive when following two conditions are true
about the problem.
\vspace{-0.14in}
\begin{itemize}[label=-\hspace{-0.02in},leftmargin=0.13in]
\item
There exist $z\in\Zcal$ values where evaluating $\gunc$ is cheaper than evaluating at
$\zhf$.
To this end, we will associate a \emph{known} cost function $\cost:\Zcal\rightarrow
\RR_+$.
In the hyper-parameter tuning example, $\cost(z) = \cost(N,T) = \bigO(N^2T)$.
It is instructive to think of $\zhf$ as being the most expensive fidelity,
i.e. maximiser of $\cost$, although this interpretation is not strictly
required.\hspace{-0.1in}
% It is instructive, albeit not necessary, to think of $\zhf$ as being the most expensive
% fidelity,
% i.e. maximiser of $\cost$, although this interpretation is not required.\hspace{-0.1in}
\vspace{-0.08in}
\item
Secondly, the cheap $\gunc(z,\cdot)$ evaluation gives us information about
$g(\zhf,\cdot)$. This is true if, for instance, $g$ is smooth across the fidelity space
as illustrated in Fig.~\ref{fig:fidelSpace}.
As we will describe shortly, we achieve this by modeling $\gunc$ as a Gaussian process
with an appropriate kernel for $\Zcal$.
\end{itemize}
A multi-fidelity algorithm is a sequence of query-fidelity pairs $\{(\xt,\zt)\}_{t\geq 0}$
where, at time $t$, the algorithm chooses $\zt\in\Zcal$ and $\xt\in\Xcal$ based on
previous query-fidelity-observation triples $\{(\xtt{i},\ztt{i},\ytt{i})\}_{i=1}^{t-1}$.
Here, $\yt = g(\zt,\xt) + \epsilon$ where $\EE[\epsilon] = 0$.

\textbf{Simple Regret:}
We provide bounds on the simple regret $S(\capital)$ of a multi-fidelity optimisation method
after it has spent capital $\capital$ of a resource.
Following~\citet{srinivas10gpbandits,kandasamy16mfbo} we
will aim to provide \emph{any capital} bounds, meaning that an algorithm would be expected
to do well for all values of (sufficiently large) $\capital$.
Say we have made $N$ queries to $g$ within capital $\capital$,
i.e. $N$ is the \emph{random} quantity such that
$N = \max\{n\geq 1: \sum_{t=1}^n \cost(\zt) \leq \capital\}$.
While the cheap evaluations $\gunc(z,\cdot)$, $z\neq \zhf$ are useful in guiding search 
for the optimum of $\gunc(\zhf,\cdot)$, there is no reward for optimising a cheaper
function. Accordingly we define the simple regret as,
\vspace{-0.07in}
\begin{align*}
S(\capital) \,=
\begin{cases}
\displaystyle\min_{\substack{t=\,1,\dots,N\\t\,:\,\zt = \zhf}}\;
  \funcopt - \func(\xt) % \hspace{0.01in}
    &\text{if we have queried at $\zhf$,} \\
+\,\infty & \text{otherwise.}
\\[-0.15in]
\end{cases}
\numberthis
\label{eqn:SLambdaDefn}
\end{align*}
\vspace{-0.25in}

This definition reduces to the single fidelity definition~\eqref{eqn:SnDefn} when we only
query $g$ at $\zhf$.
It is also similar to the definition in~\citet{kandasamy16mfbo}, but unlike them, we do
not impose additional boundedness constraints on $\func$ or $\gunc$.

\textbf{Assumptions:}
As we will be primarily focusing on continuous domains and fidelity spaces,
going forward we will assume w.l.o.g that $\Xcal = [0, 1]^d$ and $\Zcal = [0, 1]^p$.
We discuss non-continuous settings briefly at the end of Section~\ref{sec:analysis}.
In keeping with similar work in the \bayos literature we will assume
$\gunc\sim\GP(\zero,\kernel)$ and upon querying at $(z,x)$ we observe
$y = g(z,x) + \epsilon$ where $\epsilon\sim\Ncal(0,\eta^2)$.
$\kernel:(\Zcal\times\Xcal)^2\rightarrow \RR$ is
the prior covariance defined on the product space.
In this work, we will study exclusively $\kernel$ of the following form,
\begin{align*}
\kernel([z,x],[z',x']) \;=\;
\kernelscale\,\phiz(\|z-z'\|)\, \phix(\|x-x'\|).
\end{align*}
Here, $\kernelscale\in\RR_+$ is the scale parameter and $\phiz,\phix$ are radial kernels
defined on $\Zcal,\Xcal$ respectively.
The function $\phiz$ is a critical component in this work.
It controls the
smoothness of $\gunc$ across the fidelity space and hence determines how much
information the lower fidelities provide about $f(\cdot) = g(\zhf,\cdot)$.
For example, if we were to use a SE kernel for $\phiz$, a favourable setting for
a multi-fidelity method would be for $\phiz$ to have a large bandwidth $\hz$.
We will see that $\hz$ controls the behaviour and theoretical guarantees
of \mfgpucbs in a natural way in this instance.

For what follows we will also find it useful to define the following function
$\inffunc:\Zcal\rightarrow[0,1]$.
\begin{align*}
\inffunc(z) = \sqrt{1 - \phiz(\|z-\zhf\|)^2}
\label{eqn:inffunc}
\numberthis
\end{align*}
One interpretation of $\inffunc(z)$ is that it measures the \emph{loss} in
information about $g(\zhf,\cdot)$ when we query at $z\neq\zhf$.
That is, it is the price we have to pay, in information, for querying at a cheap
$z\neq\zhf$.
Note that $\inffunc$ increases when we move away from $\zhf$ in the fidelity space.
For the SE kernel, it can be shown $\inffunc(z) \approx \frac{\|z-\zhf\|}{\hz}$,
which, as expected depends on the bandwidth $\hz$.
For large $\hz$, this depends on 


==> archive/abstract.tex <==

\begin{abstract}
Bandit optimisation methods for black-box optimisation, such as Bayesian optimisation, 
are used in a variety of applications including hyper-parameter tuning and
experiment design.
Recently, \emph{multi-fidelity} methods have garnered
considerable attention since function evaluations have become increasingly expensive in
above applications.
Multi-fidelity methods use cheap approximations to the function of
interest to speed up the overall optimisation process.
However, most multi-fidelity methods assume only a finite number of approximations.
In many practical applications however, a continuous spectrum of approximations might be
available.
For instance, when tuning an expensive neural network, one might choose to approximate the
cross validation performance using less data $N$ and/or few training iterations $T$.
Here, the approximations arise out of a continuous $2$ dimensional space $(N,T)$.
In this work, we develop a Bayesian optimisation method, \boca, for this setting.
We characterise its theoretical properties and show that it achieves better regret than
than strategies which ignore the approximations.
\bocas outperforms several other baselines in synthetic and real experiments.
\end{abstract}


==> archive/appAnalysis.tex <==

\section{Analysis}
\label{sec:analysis}

\begin{definition}(Maximum Information Gain~\citep{srinivas10gpbandits})
Let $f\sim \GP(\zero, \phix)$.
Consider any $A\subset\RR^d$ and
let $A' = \{x_1, \dots, x_n\} \subset A$ be a finite subset.
Let $f_{A'}, \epsilon_{A'}\in\RR^n$ such that $(f_{A'})_i=f(x_i)$ and
$(\epsilon_{A'})_i\sim\Ncal(0,\eta^2)$.
Let $y_{A'} = f_{A'}+\epsilon_{A'}$.
Denote the Shannon Mutual Information by $I$.
The Maximum Information Gain of $A$ is
\[
\IG_n(A) = \max_{A'\subset A, |A'| = n} I(y_{A'}; f_{A'}).
\]
\label{def:infGain}
\end{definition}
\insertpostspacing




==> archive/appExperiments.tex <==

\section{Addendum to Experiments}
\label{sec:appExperiments}

\subsection{Implementation Details}
\label{sec:appIimplementation}

We describe some of our implementation details below.
\begin{itemize}[leftmargin=0.0in]
\vspace{-0.05in}
\item[]
\textbf{Domain and Fidelity space:}
Given a problem with arbitrary domain $\Xcal$ and $\Zcal$, we mapped them to
$[0,1]^d$ and $[0,1]^p$ by appropriately linear transforming the coordinates.

\item[]
\textbf{Initialisation:}
Following recommendations in~\citet{brochu12bo}
all GP methods were initialised with uniform random
queries with $\capital/10$ where $\capital$ is the capital used in the experiment.
For \gpucbs and \gpeis all queries were initialised at $\zhf$ whereas
for the multi-fidelity methods, the fidelities too were picked uniformly at random from
the available fidelities.

\item[]
\textbf{GP Hyper-parameters:}
Except in the first two experiments of Fig.~\ref{fig:toy},
the GP hyper-parameters were learned after initialisation by maximising
the GP marginal likelihood~\citep{rasmussen06gps} and then updated every 25 iterations.
We use an SE kernel for both $\phix$ and $\phiz$ and
instead of using one bandwidth for the entire fidelity space and domain, we learn
a bandwidth for each dimension separately.
We learn the kernel scale, bandwidths and noise variance using marginal likelihood.
The mean of the GP is set to be the median of the observations.

\vspace{-0.05in}
\item[]
\textbf{Choice of $\betat$:} $\betat$, as specified in Theorem~\ref{thm:regret} has unknown constants and tends to be too conservative in practice~\citep{srinivas10gpbandits}.  Following the recommendations in~\citet{kandasamy15addBO} we  set it to be of
the correct ``order''; precisely, $\betat = 0.5d\log(2\ell t + 1)$. 
Here, $\ell$ is the effective $L_1$ diamter of $\Xcal$ and is computed by scaling
each dimension by the inverse of the bandwidth of the SE kernel for that dimension.

\vspace{-0.05in}
\item[]
\textbf{Maximising $\utilt$:}
We used the \directs algorithm~\citep{jones93direct}.

\item[]
\textbf{Fidelity selection:}
Since we only worked in low dimensional fidelity spaces, the set $\candfidelst$
was constructed in practice by obtaining a finely sampled grid of $\Zcal$ and then
filtering out those which satisfied the $3$ conditions in~\eqref{eqn:candfidelst}.
In the second condition of~\eqref{eqn:candfidelst}, the threshold $\gamma(z)$ can
be multiplied up to a constant factor, i.e $c\gamma(z)$ without affecting our theoretical
results.
In practice, we started with $c=1$ but we updated it every 20 iterations via the following
rule: if the algorithm has queried $\zhf$ more than $75\%$ of the time in the last $20$
iterations, we decrease it to $c/2$ and if it queried less than $25\%$ of the time
we increase it to $2c$.
But the $c$ value is always clipped inbetween $0.1$ and $20$.
Changing $c$ this way  resulted in slightly better performance in practice.

\end{itemize}


\subsection{Description of Synthetic Functions}
\label{sec:appSynthetic}

The following are the synthetic functions used in the paper.

\begin{itemize}[leftmargin=0.0in]

\item[]
\textbf{Currin exponential function:}
The domain is the two dimensional unit cube $\Xcal = [0,1]^2$ and the fidelity 
was $\Zcal = [0, 1]$ with $\zhf = 1$.
We used $\cost(z) = 0.1 + z^2$ and,
\begin{align*}
\gunc(z, x) &= \left(1-0.1(1-z)\exp\left(\frac{-1}{2x_2}\right)\right)
  \left(\frac{2300x_1^3 + 1900x_1^2 + 2092x_1 + 60}{100x_1^3 + 
  500x_1^2 + 4x_1 + 20}\right).
\end{align*}

\item[]
\textbf{Hartmann functions:}
We used 
$g(z,x) = \sum_{i=1}^4 (\alpha_i - \alpha'_i(z)) \exp\big( -\sum_{j=1}^3 A_{ij}
(x_j-P_{ij})^2\big)$.
Here $A, P$ are given below for the $3$ and $6$ dimensional cases and
$\alpha = [1.0, 1.2, 3.0, 3.2]$.
Then $\alpha'_i$ was set as $\alpha'_i(z) = 0.1(1 - z_i)$ if $i\leq p$ for
$i=1,2,3,4$.
We constructed the $p=4$ and $p=2$ Hartmann functions for the $3$ and $6$ dimensional
cases respectively this way.
When $z = \zhf = \one_p$, this reduces to the usual Hartmann function commonly used
as a benchmark in global optimisation.
% The $M$\ssth fidelity function is
% $\funcM(x) = \sum_{i=1}^4 \alpha_i \exp\big( -\sum_{j=1}^3 A_{ij}
% (x_j-P_{ij})^2\big)$ where $A, P\in\RR^{4\times 3}$ are fixed matrices given below and
% $\alpha = [1.0, 1.2, 3.0, 3.2]$. For the lower fidelities we use the same form except
% change $\alpha$ to $\alpha^{(m)} = \alpha + (M-m)\delta$ where $\delta = [0.01, -0.01,
% -0.1, 0.1]$ and $M=3$. The domain is $\Xcal = [0,1]^3$.

For the $3$ dimensional case we used $\cost(z) = 0.05 + (1 - 0.05)z_1^3z_2^2$ and,
\[
A = 
\begin{bmatrix}
3 & 10 & 30 \\
0.1 & 10 & 35 \\
3 & 10 & 30 \\
0.1 & 10 & 35 
\end{bmatrix},
\quad
P = 10^{-4} \times
\begin{bmatrix}
3689 & 1170 & 2673 \\
4699 & 4387 & 7470 \\
1091 & 8732 & 5547 \\
381 & 5743 & 8828
\end{bmatrix}.
\]
For the $3$ dimensional case we used $\cost(z) = 0.05 + (1 -
0.05)z_1^3z_2^2z_3^{1.5}z_4^{1}$ and,
\[
A = 
\begin{bmatrix}
10 & 3 & 17 & 3.5 & 1.7 & 8 \\
0.05 & 10 & 17 & 0.1 & 8 & 14 \\
3 & 3.5 & 1.7 & 10 & 17 & 8 \\
17 & 8 & 0.05 & 10 & 0.1 & 14 
\end{bmatrix},
\;\;
P = 10^{-4} \times
\begin{bmatrix}
1312 & 1696 & 5569 &  124 & 8283 & 5886 \\
2329 & 4135 & 8307 & 3736 & 1004 & 9991 \\
2348 & 1451 & 3522 & 2883 & 3047 & 6650 \\
4047 & 8828 & 8732 & 5743 & 1091 &  381 \\
\end{bmatrix}.
\]




\item[]
\textbf{Borehole function:}
This function was taken from~\citep{xiong13highAccuracy}.
We first let,
\begin{align*}
\func_2(x) &= \frac{2\pi x_3(x_4-x_6)}
  {\log(x_2/x_1) \left(1 + \frac{2x_7x_3}{\log(x_2/x_1)x_1^2x_8} +
    \frac{x_3}{x_5} \right)}, \\
\func_1(x) &= \frac{5 x_3(x_4-x_6)}
  {\log(x_2/x_1) \left(1.5 + \frac{2x_7x_3}{\log(x_2/x_1)x_1^2x_8} +
    \frac{x_3}{x_5} \right)}. 
\end{align*}
Then we define $g(z,x) = z\func_2(x) + (1-x)\func_1(x)$.
The domain of the function is $\Xcal = [0.05, 0.15; 100, 50K; 63.07K, 115.6K;$
$990, 1110; 63.1, 116; 700, 820;$ $1120, 1680; 9855, 12045]$
and $\Zcal=[0,1]$ with $\zhf = 1$.
As the cost function we used $\cost(z) = 0.1 + z^{1.5}$.
% We first linear transform the variables to lie in $[0,1]^8$.

\item[]
\textbf{Branin function:}
We use the following function where $\Xcal=[[-5, 10], [0, 15]]^2$ and $\Zcal=[0,1]^3$.
\[
g(z,x) = a(x_2 - b(z_1)x_1^2 + c(z_2)x_1 - r)^2 + s(1-t(z))cos(x_1) + s,
\]
where $a = 1$, $b(z_1)=5.1/(4\pi^2) - 0.01(1-z_1)$
$c(z_2) = 5/\pi - 0.1(1-z_2)$, $r=6$, $s=10$ and $t(z_3)=1/(8\pi) + 0.05(1-z_3)$.
At $z=\zhf = \one_p$, this becomes the standard Branin function used as a benchmark in
global optimisation.
As the cost function we used $\cost(z) = 0.05 + z_1^{3}z_2^{2}z_3^{1.5}$.


\end{itemize}



% \subsection{Details on the Real Experiments}



==> archive/conclusion.tex <==


\section{Conclusion}
\label{sec:conclusion}


==> archive/experiments.tex <==

\section{Experiments}
\label{sec:experiments}

We compare \bocas to the following four baselines: 
\gpucb, the \gpeis criterion in \bayo~\citep{jones98expensive}, 
\mfgpucbones from~\citet{kandasamy16mfbo} and
\mfsko: the multi-fidelity sequential kriging optimisation method
from~\citet{huang06mfKriging}.
All methods are based on GPs.
The first two are not multi-fidelity methods, while the last two are finite multi-fidelity
methods\footnote{%
To our knowledge, the only other work that applies to continuous approximations
is~\citet{klein2015towards} which was developed specifically for hyper-parameter tuning.
Further, their implementation is not made available and is not straightforward to
implement.
}.
For the latter,

In all our experiments we use the SE kernel for the GPs.
We have described some implementation details for all these methods in
Appendix~\ref{sec:appImplementation}.


\subsection{Synthetic Experiments}
\label{sec:synthetic}

\insertToyResultsFigure

The results for the first set of synthetic experiments are given in Fig.~\ref{fig:toy}.
The title of each figure states the function used, and the dimensionalities $p,d$ of the
fidelity space and domain.
In all case, the fidelity space was taken to be $\Zcal=[0,1]^p$ with
$\zhf = \one_p = [1,\dots,1]\in\RR^p$
being the most expensive fidelity.
For \mfgpucbones and \mfsko, we used $3$ fidelities ($2$ approximations) where the
approximations were obtained at $z=0.333\one_p$ and $z=0.667\one_p$ points in the fidelity
space.
To reflect the setting in our experiments, we add Gaussian noise to the function value
when observing $g$ at any $(z,x)$.
This makes the problem more challenging than standard global optimisation problems
where function evaluations are not noisy.
The functions $g$, the cost functions $\cost$ and the noise variances $\eta^2$ are given
in Appendix~\ref{sec:appExperiments}.

The first two figures in Fig.~\ref{fig:toy} are simple sanity checks.
In both cases, $\Zcal=[0,1]$ and $\Xcal=[0,1]$ and the functions were sampled from GPs. 
The GP was made known to all methods which used them in picking the next point.
In the first figure, we used an SE kernel for $\phix$ with bandwidth 

In the remaining experiments, we use some standard benchmarks for global optimisation.
We modify them to obtain the function $g$ and add noise to the observations.
As the kernel and other GP hyper-parameters are unknown, we learn them by maximising
the marginal likelihood every $25$ iterations.
This is a common heuristic used in the \bayo{} literature.
We outperform all methods on all problems
except in the case of the Borehole function where \mfgpucbones does better.


\subsection{Maximum Likelihood Estimation with Type Ia Supernovae}
\label{sec:sn}

\subsection{Support Vector Classification with $20$ news groups}
\label{sec:sn}

\insertRealResultsFigure



==> archive/figureHash.tex <==

\newcommand{\imarrwthree}{2.24in}
\newcommand{\imhspthree}{-0.10in}
\newcommand{\imtextspace}{-0.15in}
\newcommand{\imsinglecol}{2.495in}
\newcommand{\imcaptionspace}{-0.1in}

\newcommand{\insertFigFidelSpace}{
\begin{figure}
\centering
\includegraphics[width=2.2in]{figs/fidel_space}
\vspace{\imcaptionspace}
\caption{\small
\label{fig:fidelSpace}
$g:\Zcal\times\Xcal\rightarrow\RR$ is a function defined on the product space of the
fidelity space $\Zcal$ and domain $\Xcal$.
The purple line is $f(x) = g(\zhf, x)$.
We wish to find the maximiser $\xopt = \argmax_{x\in\Xcal} f(x)$.
The multi-fidelity framework is attractive when $g$ is smooth across $\Zcal$ as
illustrated in the figure.
\vspace{\imtextspace}
}
\end{figure}
}


\newcommand{\insertFigBWSample}{
\begin{figure}
\centering
\includegraphics[width=1.8in]{figs/gp_bw_sample}
\vspace{\imcaptionspace}
\caption{\small
\label{fig:gpBWSample}
Samples drawn from a GP with $0$ mean and SE kernel with bandwidths $h=0.1,h=0.15,0.5$.
Samples tend to be smoother across the domain for large bandwidths.
\vspace{\imtextspace}
}
\end{figure}
}


\newcommand{\insertToyResultsFigure}{
\begin{figure*}
\centering
\hspace{\imhspthree}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/gp} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/gp_bad} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/currin_exp} \hspace{\imhspthree}
} \\[\imcaptionspace]
\hspace{\imhspthree}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/hartmann3} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/hartmann6} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/hartmann6} \hspace{\imhspthree}
} \\[\imcaptionspace]
\caption[]{\small
The simple regret $S(\capital)$ against capital $\capital$ on $6$ synthetic problems.
The title states the function used, and the fidelity and domain dimesions.
For the first two figures we used capital $30\cost(\zhf)$, therefore a method which
only queries at $g(\zhf,\cdot)$ can make at most $30$ evaluations.
For the third figure we used $50\cost(\zhf)$, for the fourth $100\cost(\zhf)$ and for
the last $200\cost(\zhf)$ to reflect the dimensionality $d$ of $\Xcal$.
The curves for the multi-fidelity methods start mid-way since they have not queried
at $\zhf$ up until that point.
All curves were produced by averaging over $20$ experiments and the error bars
indicate one standard error.
\vspace{\imtextspace}
\label{fig:toy}
}
\end{figure*}
}




\newcommand{\insertRealResultsFigure}{
\begin{figure*}
\centering
\hspace{\imhspthree}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/branin} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/branin} \hspace{\imhspthree}
}
\subfigure{
  \includegraphics[width=\imarrwthree]{figs/branin} \hspace{\imhspthree}
} \\[\imcaptionspace]
\caption[]{\small
\vspace{\imtextspace}
\label{fig:real}
}
\end{figure*}
}


==> archive/intro.tex <==

\section{Introduction}
\label{sec:intro}

Many tasks in scientific and engineering applications can be framed as \emph{bandit
optimisation} problems, where we need to sequentially evaluate a noisy
black-box function $\func:\Xcal\rightarrow\RR$ with the goal of finding its optimum.
Some applications include hyper-parameter tuning in machine learning~\citep{%
snoek12practicalBO,hutter11smac}, optimal policy search~\citep{lizotte07automaticGait,
martinez07robotplanning} and scientific experiments~\citep{parkinson06wmap3,gonzalez14gene}.
Typically, in such applications, each function evaluation is expensive and historically
the bandit literature has focused on developing methods for finding the optimum
while keeping the number of evaluations to $\func$ at a minimum.

However, with increasingly expensive experiments, conventional methods have become
infeasible as a significant cost needs to be expended before we can learn anything
about $\func$.
As a result, \emph{multi-fidelity} optimisation methods have recently gained attention.
As the name suggests, these methods assume that we have access to lower fidelity
approximate functions to $\func$ which can be evaluated instead of $\func$.
The lower the fidelity, the cheaper the evaluation, but it provides less accurate
information about $\func$.
For example, when optimising the configuration of an expensive real world robot,
its performance can be approximated using cheap computer simulations.
The goal is to use the cheap approximations to guide search for the optimum of $\func$,
and reduce the overall cost of optimisation.
However, most multi-fidelity work assume only a finite number of approximations to
$\func$.
In this paper, we study multi-fidelity optimisation when there is access to a continuous
spectrum of approximations.



To motivate this,
consider tuning a classification algorithm over a space of hyper-parameters $\Xcal$
by maximising a validation set accuracy. 
The algorithm is to be trained using $\Nmax$
data points via an iterative algorithm for $\Tmax$ iterations.
However, we wish to use fewer training points $N<\Nmax$ and/or fewer iterations
$T<\Tmax$ to approximate the validation accuracy.
We can view validation accuracy as a function
$g:[1,\Nmax]\times[1,\Tmax]\times\Xcal\rightarrow\RR$ where evaluating $g(N,T,x)$
requires training the algorithm with $N$ points for $T$ iterations with the
hyper-parameters $x$.
If the training complexity of the algorithm is quadratic in data size and linear in the
number of iterations, then the cost of this evaluation is $\lambda(N,T) = \bigO(N^2T)$.
Our goal is to find the optimum when $N=\Nmax$, and $T=\Tmax$,
% i.e.  $\xopt = \argmax_{x\in\Xcal} g(\Nmax,\Tmax, x)$.
i.e.  we wish to maximise $\func(x) = g(\Nmax,\Tmax, x)$.

In this setting, the approximations are best viewed as coming from a continuous $2$
dimensional \emph{fidelity space}, namely $[1, \Nmax]\times[1,\Tmax]$.
% Since querying $g$ at $N,T$ values less than $\Nmax,\Tmax$ costs less, we are
% tempted to use such queries in the hope that we may
Since querying $g(N,T,\cdot)$ at $N,T$ less than $\Nmax,\Tmax$ costs less, we are
tempted to use such queries in the hope that we may
learn about $g(\Nmax, \Tmax,\cdot)$ cheaply and consequently
optimise it using less overall cost.
This is, in fact, the case with many machine learning algorithms where cross
validation curves tend to vary smoothly with data set size and number of iterations.
Then we may use cheap low fidelity experiments with small $(N, T)$ to discard bad regions
of the hyper-parameter space and deploy expensive high fidelity experiments with large
$(N,T)$ only in a small but promising region of $\Xcal$.
Our proposed algorithm exhibits precisely this behaviour. 

Continuous approximations also arise in
simulation studies -- where simulations can be carried out at varying levels of granularity,
on-line advertising -- where the display of an ad can be controlled by various continuous
parameters such as display time or target audience, and various other
experiment design tasks.
In fact, in many papers on multi-fidelity optimisation, the finite approximations were
obtained by discretising
a continuous space~\citep{kandasamy16mfbo,huang06mfKriging}.
Here, we study a \bayo{} technique that is directly designed for continuous fidelity
spaces and could potentially be applied to more general spaces.
\textbf{Our contributions are as follows.}
\vspace{-0.09in}
\begin{enumerate}
\item A novel setting and model for multi-fidelity optimisation with continuous
approximations using Gaussian process (GP) assumptions.
We develop a novel algorithm, \boca, for this setting.
\vspace{-0.09in}
\item A theoretical analysis characterising the behaviour and regret bound for \boca.
\vspace{-0.09in}
\item Empirically we demonstrate that \bocas outperforms other single and multi-fidelity
  methods on a series of synthetic problems, and real problems in hyper-parameter tuning
  and computational astrophysics.
%   Our python implementation will be made publicly 
\end{enumerate}


\vspace{-0.07in}
\subsection*{Related Work}
\vspace{-0.07in}

Bayesian optimisation (\bayo), refers to a suite of techniques for bandit optimisation
which use a prior belief distribution for $\func$.
While there are several techniques for
BO~\citep{mockus94bo,jones98expensive,thompson33sampling,lobato14pes},
our work will build on the 
Gaussian process upper confidence bound (\gpucb) algorithm
of~\citet{srinivas10gpbandits}.
\gpucbs models $\func$ as a GP and uses upper confidence bound (UCB)~\citep{auer03ucb}
techniques to determine the next point for evaluation.

\bayo{} techniques have been used in developing multi-fidelity optimisation methods
in various applications such as hyper-parameter tuning and industrial
design~\citep{huang06mfKriging,swersky2013multi,klein2015towards,forrester07cokriging,%
poloczek2016multi}.
However, these methods are either problem specific and/or only use a finite
number of fidelities.
Further, none of them come with theoretical underpinnings.
Recent work has studied multi-fidelity methods for specific problems 
such as hyper-parameter tuning, active learning and
reinforcement learning%
~\citep{agarwal2011oracle,sabharwal2015selecting,cutler14mfsim,zhang15weakAndStrong,%
li2016hyperband}.
While some of the above tasks can be framed as optimisation problems, the methods
themselves are specific to the problem considered.
Our method is more general as it applies to any bandit optimisation task.


Perhaps the closest work to us is that of~\citet{kandasamy16mfbo,kandasamy16mfbandit}
who developed \mfgpucbones assuming a finite number of approximations to $\func$.
% This line of work was important as it provided the first theoretical guarantees for
% multi-fidelity optimisation.
While this line of work was the first to provide theoretical guarantees for
multi-fidelity optimisation, it has two important shortcomings.
First, they make strong assumptions, particularly a uniform bound on the
difference between the expensive function and an approximation.
This does not allow for instances where an approximation might be good at certain regions
but not at the other.
In contrast our treatment between the fidelities is probabilistic which is robust
to such cases.
Second, their model does not allow sharing information between approximations; each
approximation is treated independently.
In addition to not uti
Not only is this wasteful because lower fidelities can provide useful information about
higher fidelities, it also means that the algorithm might perform poorly if the fidelities
are not designed properly.
We demonstrate this with an experiment in Section~\ref{sec:experiments}.
On the other hand, our model allows sharing information across the fidelity space in a
natural way.
In addition, we can also handle continuous approximations whereas their method is strictly
for a finite number of approximations.
That said, \mfgpucbtwos inherits a key intuition from \mfgpucbone,
% \todo{we don't need ``-I'' anymore right? Not reading the intro part too closely yet}
% first select the next point for evaluation using an upper confidence bound strategy;
which is to choose a fidelity only if we have controlled the uncertainty at all lower
fidelities.
% However, in addition to dealing with continuous approximations, we also differ from%
% ~\citet{kandasamy16mfbo} fundamentally in our model assumptions.
Besides this, the mechanics
of our algorithm and the analysis techniques are considerably different.
As we proceed, we will draw further comparisons to~\citet{kandasamy16mfbo}.



==> archive/method.tex <==

\section{\mfgpucbtwo}
\label{sec:mfgpucb}

% We now present our \mfgpucbtwos algorithm.
\mfgpucbtwos is a sequential strategy to select a domain point $\xt\in\Xcal$ and
fidelity $\zt\in\Zcal$ at time $t$ based on previous observations.
At time $t$, we will first
construct an upper confidence bound for the function $\func$ we wish to optimise.
It takes the form,
\begin{align*}
\utilt(x) = \mutmo(x) + \betath \sigmatmo(x).
\numberthis
\label{eqn:mfucb}
\end{align*}
Recall from~\eqref{eqn:munsigman} that $\mutmo,\sigmatmo$ are the posterior mean and
standard deviation of $\func$,
i.e. $\gunc$ restricted to $\zhf$, using the observations from the previous $t-1$ time
steps.
We will specify $\betat$ in Section~\ref{sec:theory}.
Following other UCB algorithms, our next point $\xt$ in the domain $\Xcal$ for evaluating
$\gunc$ is a maximiser of $\utilt$, i.e. $\xt \in \argmax_{x\in\Xcal} \utilt(x)$.

Next, we need to determine the fidelity $\zt\in\Zcal$ to query $g$.
For this we will first select a subset $\candfidelst(\xt)$ of $\Zcal$ as follows,
% \begin{align*}
% \candfidelst(\xt) =
% %   \{\zhf\}\cup\big
%     \bigg\{z\in\Zcal\;:\;\; &\cost(z) < \cost(\zhf), \\[-0.10in]
%     &\tautmo(z,\xt) >
%       \sqrt{\kernelscale}\bigg(\hspace{-0.02in}\frac{\cost(z)}{\cost(\zhf)}
%         \hspace{-0.02in}\bigg)^{\frac{1}{d'}}
%         \inffunc(z), \\
%     &\inffunc(z) > \frac{\inffunc(\diamz) }{\betath}
%       \bigg\}.
% \numberthis\label{eqn:candfidelst}
% \end{align*}
\begin{align*}
&\candfidelst(\xt) = 
%   \{\zhf\}\cup\big
    \bigg\{z\in\Zcal\,:\,\;\cost(z) < \cost(\zhf),
    \quad\tautmo(z,\xt) > \gamma(z), \\
    &\hspace{1.25in}\inffunc(z) > \frac{\inffunc(\diamz) }{\betath}
      \bigg\}, 
\numberthis\label{eqn:candfidelst}
\\[0.05in]
&\textrm{where } \quad\gamma(z) =\,
      \sqrt{\kernelscale}\;
        \inffunc(z)\;
        \bigg(\hspace{-0.02in}\frac{\cost(z)}{\cost(\zhf)}
        \hspace{-0.02in}\bigg)^{\frac{1}{d+p+2}}
\,.
\end{align*}
Here, $\inffunc$ is the information gap function in~\eqref{eqn:inffunc},
$\tautmo$ is the posterior standard deviation of $g$,
and $\diamz = \argmax_{z\in\Zcal}\|z-\zhf\|$.
When $\Zcal=[0,1]^p$, $\diamz \leq \sqrt{p}$.
We filter out the fidelities we consider at time $t$ using three conditions as
specified above.
We elaborate on these conditions in more detail in Section~\ref{sec:fidelSelection}.
If $\candfidelst$ is not empty, we choose the cheapest fidelity in this
set, i.e. $\zt \in \argmin_{z\in\candfidelst}\cost(z)$.
If $\candfidelst$ is empty, we choose $\zt = \zhf$.
% Otherwise, we choose $\zt = \zhf$.

We have summarised the resulting procedure below in Algorithm~\ref{alg:mfgpucbtwo}.
An important advantage of \mfgpucbtwos is that it only requires specifying
the GP hyper-parameters for $\gunc$ such as the kernel $\kernel$.
In practice, this can be achieved by various effective heuristics such as maximising the
GP marginal likelihood or cross validation which are standard in most \bayos{} methods.
In contrast, \mfgpucbones of~\citet{kandasamy16mfbo} requires tuning several other
hyper-parameters.

\insertAlgoMFGPUCBTwo

\subsection{Fidelity Selection Criterion}
\label{sec:fidelSelection}

We will now provide an intuitive justification for the three conditions in the
 selection criterion for $\zt$, specifically ~\eqref{eqn:candfidelst}.
Recall that we query $\zhf$ only if $\candfidelst(\xt)$ is empty.
The first condition, $\cost(z) < \cost(\zhf)$ is fairly obvious;
since we wish to optimise $g(\zhf, \cdot)$ and since we are not rewarded for queries at
other fidelities, there
is no reason to consider fidelities that are more expensive than $\zhf$. 

The second condition, $\tautmo(z,\xt) > \gamma(z)$ says that we will only consider
fidelities where the posterior
variance is larger than a threshold
$\gamma(z) = \sqrt{\kernelscale}\inffunc(z)(\cost(z)/\cost(\zhf))^{1/(p+d+2)}$,
 which depends critically on two
quantities, the cost function $\cost$ and the information gap $\inffunc$.
First, a reasonable multi-fidelity strategy should be inclined to query cheap
fidelities and learn about $\gunc$ before querying expensive fidelities.
This is the case with \mfgpucbtwo; as $\gamma(z)$ decreases with $\cost(z)$, it becomes
easier for cheap $z$ to satisfy $\tautmo(z,\xt)>\gamma(z)$ and be included in
$\candfidelst$ at time $t$.
As we choose $\zt$ to be the minimiser of $\cost$ in $\candfidelst$,
a cheaper fidelity will always be chosen over expensive ones if included in $\candfidelst$.
Secondly, if $z$ is far away from $\zhf$ it contains less information
about $g(\zhf,\cdot)$.
A reasonable strategy should be discouraged from making such queries.
This is precisely the role of the information gap $\inffunc$ which is increasing with
$\|z-\zhf\|$.
As we move away from $\zhf$, $\gamma(z)$ increases and
it becomes harder to satisfy $\tautmo(z,\xt)>\gamma(z)$.
Therefore, $z$ far away from $\zhf$ are  less likely
to be included in $\candfidelst(\xt)$ and be considered for evaluation.
Our analysis reveals that setting $\gamma$ as in~\eqref{eqn:candfidelst} is a
reasonable way to manage this trade off between cost and information where
cheaper fidelities cost less, but provide less accurate information about the
function $\func$ we wish to optimise.

To provide more intuition for the second condition,
recall that for the SE kernel, $\inffunc(z) \approx \|z-\zhf\|/\hz$ where $\hz$ is the
bandwidth of $\phiz$.
If $\gunc$ is very smooth across $\Zcal$, then the lower fidelities provide more
information about $g(\zhf,\cdot)$.
One should expect a reasonable strategy
to exploit such information considerably as it is cheaper.
Indeed, large $\hz$ reduces the threshold $\gamma(z)$ across the
entire $\Zcal$, causing $\candfidelst$ to be nonempty and \mfgpucbtwos to
consider lower fidelities extensively before proceeding to $\zhf$.
On the other hand, if $\hz$ is small and $\gunc$ is not smooth across $\Zcal$, the
threshold $\gamma(z)$ will be large for all $z$. 
Then $\candfidelst$ vanishes fast and the algorithm will aggressively
skip lower fidelities and proceed to $\zhf$.
Thus, this behaviour of \mfgpucbtwos is sensible in the SE kernel case.
It is worth noting that the second condition is similar in
spirit to~\citet{kandasamy16mfbo} where they proceed from a lower to higher
fidelity only when the lower fidelity variance is smaller than a threshold.
However, while they treat the threshold as a hyper-parameter, we are able to explicitly
specify theoretically motivated values for it.


Finally, the third condition in~\eqref{eqn:candfidelst},
$\inffunc(z) > \inffunc(\diamz)/\betath$, 
says that we should only pick
fidelities where the information gap $\inffunc$ is large.
Since $\inffunc$ is increasing as we move away from
$\zhf$, it says we will only consider fidelities outside a neighbourhood of $\zhf$.
Such a condition is necessary when dealing with continuous fidelities to
prevent pathological situations where an algorithm might get arbitrarily close to
$\zhf$ but not actually query \emph{at} $\zhf$.
This condition breaks the continuum and forces \bocas to pick $\zhf$ instead of
querying very close to it.
Observe that as $\betat$ is increasing with $t$, this neighborhood is shrinking with time
and therefore the algorithm will eventually have the opportunity to evaluate fidelities
close to $\zhf$.
Next, we describe our theoretical results.

\input{theory}


% \subsection{Practical Implementation}
% \label{sec:implementation}


% \subsection{Beyond Continuous Fidelity spaces and Domains}
% \label{sec:extensions}

\textbf{Extensions:}
While we have focused on continuous $\Zcal$ due to their wide ranging
practical applications, many of the ideas here can be extended to other settings.
If $\Zcal$ is a discrete subset of $[0,1]^p$ our ideas here can be extended
straightforwardly.
We reiterate that this will \emph{not} be the same as the finite fidelity
\mfgpucbones algorithm  since the assumptions are significantly different.
In particular,~\citet{kandasamy16mfbo} are not able to effectively share
information across fidelities as we do.
We also believe that Algorithm~\ref{alg:mfgpucbtwo} can be extended to arbitrary fidelity
spaces $\Zcal$ as long as a kernel can be defined over $\Zcal$.
% Another avenue for future work would be to study different choices for
% $\Zcal$ kernel where 
% These questions are left for future work.
% In particular when $\Xcal$ is a discrete set, the analysis can be extended in a
% straightforward way.
Our results can also be straightforwardly extended for discrete domains $\Xcal$
and various kernel choices for $\phix$ by mimicking the proofs
from~\citet{srinivas10gpbandits}.
As with most nonparametric methods, \mfgpucbtwos scales poorly with
dimension due to the dependence on $\IGn$.
Due to this reason, we also confine our experiments to small $p,d$.
This can be alleviated by assuming additional structure on
$\func,\gunc$~\citep{djolonga13highdimbandits,kandasamy15addBO}.




==> archive/prelims.tex <==
\section{Preliminaries}
\label{sec:prelims}

% \subsection{A Review of Gaussian processes and \gpucb}
\subsection{Some Background Material}
\label{sec:prelims}

\textbf{Gaussian processes:}
A GP over a space $\Xcal$ is a random process describing functions from $\Xcal$ to $\RR$.
It is characterised by a mean function $\mu:\Xcal\rightarrow\RR$ and
a covariance kernel $\kernel:\Xcal^2\rightarrow\RR$.
If $\func\sim\GP(\mu,\kernel)$, then $f(x)$ is distributed normally
$\Ncal(\mu(x), \kernel(x,x))$ for all $x\in\Xcal$.
Suppose we are given $n$ observations from this GP, $\Dcal_n=\{(x_i, y_i)\}_{i=1}^n$ where
$x_i\in\Xcal$, $y_i = \func(x_i) + \epsilon_i \in\RR$ and $\epsilon_i\sim\Ncal(0,\eta^2)$.
Then the posterior process $\func|\Dcal_n$ is also a GP with some mean $\mu_n$ and
covariance $\kernel_n$, where
\begin{align*}
\hspace{-0.05in}
\mu_n(x) &= \kb^\top\Delta^{-1}Y, \hspace{0.35in}
\numberthis \label{eqn:gpPost} \\
\kernel_n(x,x') &= \kernel(x,x') - \kb^\top\Delta^{-1}\kb'.
\hspace{0.05in}
\end{align*}
Here, $Y\in\RR^n$ with $Y_i=y_i$,
$\kb,\kb'\in\RR^n$ with $\kb_i =
\kernel(x,x_i),\kb'_i=\kernel(x',x_i)$ and
$\Delta = \Kb + \eta^2I \in \RR^{n\times n}$ where
$\Kb_{i,j} = \kernel(x_i,x_j)$~\citep{rasmussen06gps}.
% We refer readers unfamiliar with GPs to chapter 2 of~\citet{rasmussen06gps} for
% the formulae for $\mu_n,\kernel_n$ and other properties of GPs.

\textbf{Radial kernels:}
Radial kernels are commonly used in the prior covariance of GPs;
% The squared exponential (SE) kernel and \matern{} kernels, which are popularly used in
% practice, are radial kernels.
some examples are the squared exponential (SE) and \matern{} kernels~\citep{rasmussen06gps}.
When using a radial kernel,
the prior covariance can be written as $\kernel(x,x') = \kernelscale\phi(\|x-x'\|)$ and
depends only on the distance between $x$ and $x'$.
Here, the scale parameter $\kernelscale$ 
captures the magnitude $\func$ could deviate from $\mu$.
The radial kernel, $\phi:\RR_{+}\rightarrow\RR_+$, is a decreasing function with
$\|\phi\|_\infty = \phi(0) = 1$.
In this paper, we will use the SE kernel in a running example to convey the
intuitions in our methods. 
For the SE kernel, $\phi(r) = \radialh(r) = \exp(-r^2/(2h^2))$, where $h\in\RR_+$ is
the bandwidth parameter and controls the smoothness of the GP.
% It is well known that 
When $h$ is large, the samples drawn from the GP tend to
be smoother as illustrated in Fig.~\ref{fig:gpBWSample}.
We will reference this observation frequently in the text.

\insertFigBWSample

\textbf{\gpucb:}
The Gaussian Process Upper Confidence Bound (\gpucb) algorithm
of~\citet{srinivas10gpbandits}  is a method for bandit optimisation,
which, like many other \bayos methods, models $\func$ as a sample from a Gaussian process.
At time $t$, the next point $\xt$ for evaluating $\func$ is chosen via the following
procedure.
First, we construct an upper confidence bound
$\utilt(x) = \mutmo(x) + \betath \sigmatmo(x)$ for the GP. 
$\mutmo$ is the posterior mean of the GP conditioned on the previous $t-1$ evaluations
and $\sigmatmo$ is the posterior standard deviation.
Then the next point is chosen by maximising $\utilt$, i.e.
$\xt=\argmax_{x\in\Xcal}\utilt(x)$.
The $\mutmo$ term encourages an \emph{exploitative} strategy -- in that we want to query
regions where we already believe  $\func$ is high -- and $\sigmatmo$ encourages
an \emph{exploratory} strategy -- in that we want to query where we are uncertain
about $\func$ so that we do not miss regions which have not been queried yet.
$\betat$, which is typically increasing with $t$, controls the trade-off between
exploration and exploitation.


\subsection{Problem Set Up}
\label{sec:prelims}

% In stochastic bandit optimisation, our goal is to maximise a function
Our goal in bandit optimisation is to maximise a function
$\func:\Xcal\rightarrow \RR$, over a domain $\Xcal$.
When we evaluate $\func$ at $x\in\Xcal$ we observe $y=\func(x) + \epsilon$ where
$\EE[\epsilon] = 0$.
Let $\xopt \in \argmax_{x\in\Xcal}\func(x)$ be a maximiser of $\func$ and
$\funcopt = \func(\xopt)$ be the maximum value.
% $\func$ is accessible only via noisy point evaluations and has no gradient information.
An algorithm for bandit optimisation is a sequence of points $\{\xt\}_{t\geq0}$, where
at time $t$, the algorithm chooses to evaluate $\func$ at $\xt$ based on previous queries
and observations $\{(\xtt{i},\ytt{i})\}_{i=1}^{t-1}$.
After $n$ queries to $\func$,
its goal is to achieve small \emph{simple regret} $\Sn$, as defined below.
\begin{align*}
\Sn = \min_{t=1,\dots,n} \funcopt - \func(\xt).
\numberthis
\label{eqn:SnDefn}
\end{align*}
\textbf{Multi-fidelity Bandit Optimisation:}
In this work, we will let $\func$ be a slice of a function $\gunc$ that lies
in a larger space.
In particular, we will assume the existence of a fidelity space $\Zcal$ and a function 
$\gunc:\Zcal\times\Xcal \rightarrow \RR$ defined on the product space of the fidelity
space and domain.
The function $\func$ which we wish to maximise is related to $\gunc$ via
$\func(\cdot) = \gunc(\zhf, \cdot)$, where $\zhf\in\Zcal$.
For instance, in the hyper-parameter tuning example from Section~\ref{sec:intro},
$\Zcal = [1,\Nmax]\times[1,\Tmax]$ and $\zhf = [\Nmax, \Tmax]$.
Our goal is to find the maximiser $\xopt = \argmax_x \func(x) = \argmax_x \gunc(\zhf, x)$.
We have illustrated this set up in Fig.~\ref{fig:fidelSpace}.
In the rest of the manuscript, the term ``fidelities'' will refer to points $z$
in the fidelity space $\Zcal$.
\insertFigFidelSpace

The multi-fidelity framework is attractive when the following two conditions are true
about the problem.
\vspace{-0.10in}
% \begin{itemize}[label=-\hspace{-0.02in},leftmargin=0.13in]
\begin{enumerate}[leftmargin=0.19in]
\item
\ul{There exist fidelities $z\in\Zcal$ where evaluating $\gunc$ is cheaper than
evaluating at $\zhf$.}
To this end, we will associate a \emph{known} cost function $\cost:\Zcal\rightarrow
\RR_+$.
In the hyper-parameter tuning example, $\cost(z) = \cost(N,T) = \bigO(N^2T)$.
It is helpful to think of $\zhf$ as being the most expensive fidelity,
i.e. maximiser of $\cost$, and that $\cost(z)$ decreases as we move away from
$\zhf$. 
However, this notion is strictly not necessary for our algorithm
or results.\hspace{-0.1in}
\vspace{-0.06in}
\item
\ul{The cheap $\gunc(z,\cdot)$ evaluation gives us information about
$g(\zhf,\cdot)$.}
This is true if $\gunc$ is smooth across the fidelity space
as illustrated in Fig.~\ref{fig:fidelSpace}.
As we will describe shortly, this can be achieved by modelling $\gunc$ as a Gaussian process
with an appropriate kernel for $\Zcal$.
% \end{itemize}
\end{enumerate}
\vspace{-0.12in}

In the above set up, a multi-fidelity algorithm is a sequence of query-fidelity pairs
$\{(\zt,\xt)\}_{t\geq 0}$
where, at time $t$, the algorithm chooses $\zt\in\Zcal$ and $\xt\in\Xcal$ based on
previous fidelity-query-observation triples $\{(\ztt{i},\xtt{i},\ytt{i})\}_{i=1}^{t-1}$.
Here, $\ytt{i} = g(\ztt{i},\xtt{i}) + \epsilon$ where $\EE[\epsilon] = 0$.

\textbf{Multi-fidelity Simple Regret:}
We provide bounds on the simple regret $S(\capital)$ of a multi-fidelity optimisation method
after it has spent capital $\capital$ of a resource.
Following~\citet{srinivas10gpbandits,kandasamy16mfbo} we
will aim to provide \emph{any capital} bounds, meaning that an algorithm would be expected
to do well for \emph{all} values of (sufficiently large) $\capital$.
Say we have made $N$ queries to $g$ within capital $\capital$,
i.e. $N$ is the \emph{random} quantity such that
$N = \max\{n\geq 1: \sum_{t=1}^n \cost(\zt) \leq \capital\}$.
While the cheap evaluations at $z\neq \zhf$ are useful in guiding search 
for the optimum of $\gunc(\zhf,\cdot)$, there is no reward for optimising a cheaper
$g(z,\cdot)$. Accordingly we define the simple regret after capital $\capital$ as,
\vspace{-0.02in}
\begin{align*}
S(\capital) \,=
\begin{cases}
\displaystyle\min_{\substack{t=\,1,\dots,N\\t\,:\,\zt = \zhf}}\;
  \funcopt - \func(\xt) % \hspace{0.01in}
    &\text{if we have queried at $\zhf$,} \\
+\,\infty & \text{otherwise.}
\end{cases}
\\[-0.15in]
% \numberthis
% \label{eqn:SLambdaDefn}
\end{align*}
\vspace{-0.35in}

This definition reduces to the single fidelity definition~\eqref{eqn:SnDefn} when we only
query $g$ at $\zhf$.
It is also similar to the definition in~\citet{kandasamy16mfbo}, but unlike them, we do
not impose additional boundedness constraints on $\func$ or $\gunc$.

Before we proceed, we note that it is customary in the bandit literature to analyse
\emph{cumulative regret}. However, the definition of cumulative regret depends
on the
application at hand~\citep{kandasamy16mfbandit} and the results in this paper can be
extended to to many sensible notions of cumulative regret.
However, both to simplify exposition and since our focus in this paper is optimisation,
we stick to simple regret.

\textbf{Assumptions:}
As we will be primarily focusing on continuous and compact domains and fidelity spaces,
going forward we will assume, without any loss of generality, that $\Xcal = [0, 1]^d$ and
$\Zcal = [0, 1]^p$.
We discuss non-continuous settings briefly at the end of Section~\ref{sec:mfgpucb}.
In keeping with similar work in the Bayesian optimisation literature, we will
assume
$\gunc\sim\GP(\zero,\kernel)$ and upon querying at $(z,x)$ we observe
$y = g(z,x) + \epsilon$ where $\epsilon\sim\Ncal(0,\eta^2)$.
$\kernel:(\Zcal\times\Xcal)^2\rightarrow \RR$ is
the prior covariance defined on the product space.
In this work, we will study exclusively $\kernel$ of the following form,
\begin{align*}
\hspace{-0.1in}
\kernel([z,x],[z',x']) \,=\,
\kernelscale\,\phiz(\|z-z'\|)\, \phix(\|x-x'\|).
\label{eqn:mfkernel}
\numberthis
\end{align*}
Here, $\kernelscale\in\RR_+$ is the scale parameter and $\phiz,\phix$ are radial kernels
defined on $\Zcal,\Xcal$ respectively.
The fidelity space kernel $\phiz$ is an important component in this work.
It controls the
smoothness of $\gunc$ across the fidelity space and hence determines how much
information the lower fidelities provide about $g(\zhf,\cdot)$.
For example, suppose that $\phiz$ was a SE kernel.
A favourable setting for
a multi-fidelity method would be for $\phiz$ to have a large bandwidth $\hz$
as that would imply that $g$ is very smooth across $\Zcal$.
We will see that $\hz$ determines the behaviour and theoretical guarantees
of \mfgpucbtwos in a natural way when $\phiz$ is the SE kernel.
To formalise this, we will  define the following function
$\inffunc:\Zcal\rightarrow[0,1]$.
\begin{align*}
\inffunc(z) = \sqrt{1 - \phiz(\|z-\zhf\|)^2}
\label{eqn:inffunc}
\numberthis
\end{align*}
One interpretation of $\inffunc(z)$ is that it measures the \emph{gap} in
information about $g(\zhf,\cdot)$ when we query at $z\neq\zhf$.
That is, it is the price we have to pay, in information, for querying at a cheap fidelity.
Observe that $\inffunc$ increases when we move away from $\zhf$ in the fidelity space.
For the SE kernel, it can be shown $\inffunc(z) \approx \frac{\|z-\zhf\|}{\hz}$.
For large $\hz$, $\gunc$ is smoother across $\Zcal$ and we can expect the lower fidelities
to be more informative about $\func$;  as expected $\inffunc$ is small for large $\hz$.
If $\hz$ is small and $\gunc$ is not smooth, the loss of information $\inffunc$ is large
and lower fidelities are not as informative.

% \todo{@samy, see comment in the code below}
%%% @samy: when defining functions, dont forcibly include space. The right way to do it is to define the command as usual and call the function with trailing parentheses. This is because Latex, by default, assumes that any character following \bayos is an argument to the function \bayos, by default. This is why it messes up spaces sometimes. So, the right way to do it is to always call functions as '\bayos{}' (I have done this in this case).}

Before we present our algorithm for the above setup, we will introduce notation for the posterior GPs for $\gunc$ and $\func$.
Let $\Dcal_n = \{(\ztt{i},\xtt{i},\ytt{i})\}_{t=1}^n$ be $n$ fidelity, query,
observation values from the GP $\gunc$, where $\ytt{i}$ was observed when evaluating
$g(\ztt{i},\xtt{i})$.
We will denote the posterior mean and standard
deviation of $\gunc$ conditioned on $\Dcal_n$ by $\nutt{n}$ and $\tautt{n}$ respectively
($\nutt{n},\tautt{n}$ can be computed from~\eqref{eqn:gpPost} by replacing
$x\leftarrow[z,x]$).
Therefore $\gunc(z,x)|\Dcal_n\sim\Ncal(\nutt{n}(z,x), \tausqtt{n}(z,x))$ for all
$(z,x)\in\Zcal\times\Xcal$.
We will further denote 
\begin{align*}
\mutt{n}(\cdot) = \nutt{n}(\zhf,\cdot), \hspace{0.2in}
\sigmatt{n}(\cdot) = \tautt{n}(\zhf,\cdot),
\label{eqn:munsigman}
\numberthis
\end{align*}
to be the posterior mean and standard
deviation of $\gunc(\zhf,\cdot) = \func(\cdot)$.
It follows that $\func|\Dcal_n$ is also a GP and satisfies
$\func(x)|\Dcal_n \sim \Ncal(\mutt{n}(x), \sigmasqtt{n}(x))$ for all $x\in\Xcal$.



==> archive/tableHash.tex <==

\newcommand{\insertAlgoMFGPUCBTwo}{
% \vspace{-0.05in}
\begin{algorithm}
\textbf{Input: } kernel $\kernel$.
\vspace{-0.07in}
\begin{itemize}[leftmargin=0.23in]
\item Set $\;\;\nutt{0}(\cdot)\leftarrow\zero$,
          $\;\;\tautt{0}(\cdot)\leftarrow\kernel(\cdot,\cdot)^{1/2}$, 
          $\;\;\Dcal_0\leftarrow\emptyset$. 
\vspace{-0.05in}
\item for $t = 1, 2,\dots$
\vspace{-0.05in}
  \begin{enumerate}[leftmargin=0.23in]
  \item $\xt \leftarrow \argmax_{x\in\Xcal} \,\utilt(x)$. 
  \hfill See~\eqref{eqn:mfucb}
  \item $\zt \leftarrow \argmin_{z\in\,\candfidelst(\xt)\cup\{\zhf\}} \,\cost(z)$. 
  \hfill See~\eqref{eqn:candfidelst}
  \item $\yt \leftarrow$ Query $\gunc$ at $(\zt,\xt)$.
  \item $\Dcal_t\leftarrow\Dcal_{t-1}\cup\{(\zt,\xt,\yt)\}$.
        Update posterior mean $\nutt{t}$, and standard deviation $\tautt{t}$ conditioned on $\Dcal_t$.
%   \item \textbf{for} $m=1,\dots,M$:  \\
%     \vphantom{T} \hspace{0.1in} 
%       \textbf{if} $\betath\sigmamtmo(\xt) > \gamma$, \textbf{break}; \\
%     $\mt = m$.
%   \item $\Dcalmtt \leftarrow \Dcalmmtt{\mt}{t-1}\cup\{(\xt,\yt)\}$.
%   \item $\Dcalmt \leftarrow \Dcalmmtt{m}{t-1}$ for all $m\neq \mt$.
%   \item Obtain $\mumtt,\sigmamtt$ conditioned on $\Dcalmtt$.
  \end{enumerate}
% \vspace{-0.1in}
\end{itemize}
\vspace{-0.1in}
\caption{\hspace{0.05in}\mfgpucbtwo \label{alg:mfgpucbtwo}}
\end{algorithm}
% \vspace{-0.05in}
}


==> archive/theory.tex <==

\subsection{Theoretical Results}
\label{sec:theory}


We now present our main theoretical contributions.
In order to simplify the exposition and convey the gist of our results, we will
only present a simplified version of our theorems.
We will suppress constants, $\polylog$ terms, and other technical
details that arise due to a covering argument in our proofs.
A rigorous treatment is available in Appendix~\ref{sec:analysis}.


\textbf{Maximum Information Gain:}
Up until this point, we have not discussed much about the kernel $\phix$ of the
domain $\Xcal$.
Since we are optimising $\func$ over $\Xcal$, it is natural to expect that this
will appear in the bounds.
\citet{srinivas10gpbandits} showed that the statistical difficulty of GP bandits is
determined by the \emph{Maximum Information Gain} (\mig) which measures the maximum
information a subset of observations have about $\func$. 
We denote it by $\IGn(A)$ where $A$ is a subset of $\Xcal$ and $n$ is the number of
queries to $\func$.
We have given the technical definition of the \migs in Appendix~\ref{sec:analysis},
but for our purposes it is sufficient to know that $\IGn(A)$ depends
on the domain kernel $\phix$,
the number of times $n$ we have queried $\func$ and the volume of $A$. 
The latter dependence on $\vol(A)$ will be most important to us.
For instance, when we use an SE kernel for $\phix$, we have
$\IGn(A) \propto \vol(A)\,\logn^{d+1}$%
~\citep{srinivas10gpbandits,seeger08information}.
The simple regret $S(\capital)$ for \gpucbs after capital $\capital$ can be bounded by,
\begin{align*}
\hspace{-0.1in}
\text{Simple Regret for \gpucb:}\hspace{0.15in}
S(\capital) \lesssim 
  \sqrt{\frac{\IGnc(\Xcal)}{\ncapital}},
\label{eqn:gpucbregret}
\numberthis
\end{align*}
where $\ncapital = \floor{\capital/\cost(\zhf)}$.


In our analysis of \mfgpucbtwos we show that most queries to $\gunc$ at fidelity
$\zhf$ will be confined to a small subset of the domain $\Xcal$ which contains the
 optimum $\xopt$.
Precisely, after capital $\capital$, for all $\alpha\in(0,1)$,
there exists $\rho>0$ such that the number of queries \emph{outside} the following
set $\Xcalrho$ is less than $\ncapital^\alpha$.
\begin{align*}
\Xcalrho = \big\{x\in\Xcal\,:\, \funcopt - \func(x)
\leq 2\rho\sqrt{\kernelscale}\,\inffunc(\diamz) \big\}.
\label{eqn:Xcalrho}
\numberthis
\end{align*}
Here, $\inffunc$ is from~\eqref{eqn:inffunc} and $\diamz$ is the $L_2$
diameter of $\Zcal$. %\todo{the following lines are not very clear.}
While it is true that any optimisation algorithm would eventually query extensively
in a neighbourhood around the optimum, a strong result of the above type is
not always possible.
For e.g., the best achievable bound on the number of queries by \gpucbs for any
set that does not contain $\xopt$ is $\ncapital^{1/2}$.
The above set $\Xcalrho$ arises exclusively due to our multi-fidelity assumptions
and we are able to control the plays outside $\Xcalrho$ using information
from lower fidelities.
% and is determined by the smoothness of $\gunc$ across $\Zcal$.
As $\inffunc$ is small when $\gunc$ is smooth across $\Zcal$,  the set $\Xcalrho$ will
be small when the approximations are highly informative about $\gunc(\zhf, \cdot)$. 
To see this more clearly, we revert to the case where $\phiz$ is a SE kernel
where we have 
 $\Xcalrho \approx \{x\in\Xcal: \funcopt - \func(x) \leq 2\rho\sqrt{p}/\hz\}$.
When $\hz$ is large and $\gunc$ is smooth across $\Zcal$, $\Xcalrho$ is small 
as the right side of the inequality is smaller.
As \mfgpucbtwos confines most of its evaluations to this small set
containing $\xopt$, we will be able to achieve much better regret than \gpucb.
When $\hz$ is small and $\gunc$ is not smooth across $\Zcal$,
the set $\Xcalrho$ becomes large and the advantage of multi-fidelity
optimisation diminishes.


We now provide an informal statement of our main result below.
$\lesssim,\asymp$ will denote inequality and equality ignoring constant and
$\polylog$ terms.

\begin{theorem}[Informal, Regret of \mfgpucbtwo]
\label{thm:regret}
Let $g\sim\GP(0,\kernel)$ where $\kernel$ satisfies~\eqref{eqn:mfkernel}.
Choose $\betat \asymp d\log(t/\delta)$.
Then, for sufficiently large $\capital$ and for all $\alpha \in(0,1)$, there exists $\rho$
depending on $\alpha$ such that the following bound holds w.h.p.
\[
S(\capital) \;\lesssim\;
  \sqrt{\frac{\IGnc(\Xcalrho)}{\ncapital}}
  \;+\;
  \sqrt{\frac{\IGncalpha(\Xcal)}{\ncapital^{2-\alpha}}}
\]
\end{theorem}
In the above bound, the latter term vanishes fast due to the $\ncapital^{-(1-\alpha/2)}$
dependence.
When comparing this with~\eqref{eqn:gpucbregret},
we see that we outperform \gpucbs by a factor of
$\sqrt{\IGnc(\Xcalrho)/\IGnc(\Xcal)} \asymp \sqrt{\vol(\Xcalrho)/\vol(\Xcal)}$
asymptotically.
If $\gunc$ is smooth across the fidelity space, $\Xcalrho$ is small and
the gains over \gpucbs are significant.
If $\gunc$ becomes less smooth across $\Zcal$, the bound decays gracefully, but
we are never worse than \gpucbs up to constant factors.

Theorem~\ref{thm:regret} also has similarities to the bounds 
of~\citet{kandasamy16mfbo} who also demonstrate better regret than \gpucbs by
showing that it is dominated by queries inside a set $\Xcal'$ which contains the optimum.
However, their bounds also depend critically on certain threshold hyper-parameters
which determines the volume of $\Xcal'$ among other  terms in their regret.
The authors of that paper note that their bounds will suffer if these hyper-parameters are not
chosen appropriately, but do not provide theoretically justified methods to do so.
In contrast, many of the design choices of our method fall out naturally from
our modeling assumptions.
Beyond this analogue, our results are not comparable to~\citet{kandasamy16mfbo}
as the assumptions are very different.



==> old_method.tex <==

\section{\mfgpucbtwo: Bayesian Optimisation with Continuous Approximations}
\label{sec:mfgpucb}

% We now present our \mfgpucbtwos algorithm.
\mfgpucbtwos is a sequential strategy to select a domain point $\xt\in\Xcal$ and
fidelity $\zt\in\Zcal$ at time $t$ based on previous observations.
At time $t$, we will first
construct an upper confidence bound for the function $\func$ we wish to optimise.
It takes the form,
\begin{align*}
\utilt(x) = \mutmo(x) + \betath \sigmatmo(x).
\numberthis
\label{eqn:mfucb}
\end{align*}
Recall from~\eqref{eqn:munsigman} that $\mutmo,\sigmatmo$ are the posterior mean and
standard deviation of $\func$,
i.e. $\gunc$ restricted to $\zhf$, using the observations from the previous $t-1$ time
steps.
We will specify $\betat$ in Section~\ref{sec:theory} \todo{need a more specific pointer, hard to find}.
Following other UCB algorithms, our next point $\xt$ in the domain $\Xcal$ for evaluating
$\gunc$ is a maximiser of $\utilt$, i.e. $\xt \in \argmax_{x\in\Xcal} \utilt(x)$.

Next, we need to determine the fidelity $\zt\in\Zcal$ to query $g$.
For this we will first select a subset $\candfidelst(\xt)$ of $\Zcal$ as follows,
% \begin{align*}
% \candfidelst(\xt) =
% %   \{\zhf\}\cup\big
%     \bigg\{z\in\Zcal\;:\;\; &\cost(z) < \cost(\zhf), \\[-0.10in]
%     &\tautmo(z,\xt) >
%       \sqrt{\kernelscale}\bigg(\hspace{-0.02in}\frac{\cost(z)}{\cost(\zhf)}
%         \hspace{-0.02in}\bigg)^{\frac{1}{d'}}
%         \inffunc(z), \\
%     &\inffunc(z) > \frac{\inffunc(\diamz) }{\betath}
%       \bigg\}.
% \numberthis\label{eqn:candfidelst}
% \end{align*}
\begin{align*}
&\candfidelst(\xt) = 
%   \{\zhf\}\cup\big
    \bigg\{z\in\Zcal\,:\,\;\cost(z) < \cost(\zhf),
    \quad\tautmo(z,\xt) > \gamma(z), \\
    &\hspace{1.25in}\inffunc(z) > \frac{\inffunc(\diamz) }{\betath}
      \bigg\}, 
\numberthis\label{eqn:candfidelst}
\\[0.05in]
&\textrm{where } \quad\gamma(z) =\,
      \sqrt{\kernelscale}\;
        \inffunc(z)\;
        \bigg(\hspace{-0.02in}\frac{\cost(z)}{\cost(\zhf)}
        \hspace{-0.02in}\bigg)^{\frac{1}{d+p+2}}
\,.
\end{align*}
Here, $\inffunc$ is the information gap function in~\eqref{eqn:inffunc},
$\tautmo$ is the posterior standard deviation of $g$,
and $\diamz = \argmax_{z\in\Zcal}\|z-\zhf\|$.
When $\Zcal=[0,1]^p$, $\diamz \leq \sqrt{p}$.
We filter out the fidelities we consider at time $t$ using three conditions as
specified above.
We elaborate on these conditions in more detail in Section~\ref{sec:fidelSelection}.
If $\candfidelst$ is not empty, we choose the cheapest fidelity in this
set, i.e. $\zt \in \argmin_{z\in\candfidelst}\cost(z)$.
If $\candfidelst$ is empty, we choose $\zt = \zhf$.
% Otherwise, we choose $\zt = \zhf$.

We have summarised the resulting procedure below in Algorithm~\ref{alg:mfgpucbtwo}.
An important advantage of \mfgpucbtwos is that it only requires specifying
the GP hyper-parameters for $\gunc$ such as the kernel $\kernel$.
In practice, this can be achieved by various effective heuristics such as maximising the
GP marginal likelihood or cross validation which are standard in most \bayos{} methods.
In contrast, \mfgpucbones of~\citet{kandasamy16mfbo} requires tuning several other
hyper-parameters.

\insertAlgoMFGPUCBTwo

\subsection{Fidelity Selection Criterion}
\label{sec:fidelSelection}

We will now provide an intuitive justification for the three conditions in the
 selection criterion for $\zt$, i.e., equation~\eqref{eqn:candfidelst}.
Recall that we query $\zhf$ only if $\candfidelst(\xt)$ is empty.
The first condition, $\cost(z) < \cost(\zhf)$ is fairly obvious;
since we wish to optimise $g(\zhf, \cdot)$ and since we are not rewarded for queries at
other fidelities, there
is no reason to consider fidelities that are more expensive than $\zhf$. 

The second condition, $\tautmo(z,\xt) > \gamma(z)$ says that we will only consider
fidelities where the posterior
variance is larger than a threshold
$\gamma(z) = \sqrt{\kernelscale}\inffunc(z)(\cost(z)/\cost(\zhf))^{1/(p+d+2)}$,
 which depends critically on two
quantities, the cost function $\cost$ and the information gap $\inffunc$. As a first step towards parsing this condition, observe that a reasonable multi-fidelity strategy should be inclined to query cheap
fidelities and learn about $\gunc$ before querying expensive fidelities. Now notice that $\gamma(z)$ is defined so that it is monotonic in $\cost(z)$, therefore, it becomes
easier for a cheap $z$ to satisfy $\tautmo(z,\xt)>\gamma(z)$ and be included in
$\candfidelst$ at time $t$. Moreover, since we choose $\zt$ to be the minimiser of $\cost$ in $\candfidelst$,
a cheaper fidelity will always be chosen over expensive ones if included in $\candfidelst$. 
Secondly, if a particular fidelity $z$ is far away from $\zhf$, it probably contains less information
about $g(\zhf,\cdot)$. Again, a reasonable multi-fidelity strategy should be discouraged from making such queries. 
This is precisely the role of the information gap $\inffunc$ which is increasing with
$\|z-\zhf\|$.
As a particular fidelity $z$ moves away from $\zhf$, $\gamma(z)$ increases and
it becomes harder to satisfy $\tautmo(z,\xt)>\gamma(z)$.
Therefore, such a $z$ is less likely
to be included in $\candfidelst(\xt)$ and be considered for evaluation.
Our analysis reveals that setting $\gamma$ as in~\eqref{eqn:candfidelst} allows us to trade off between the cost and information of the fidelities available to us; 
cheaper fidelities cost less, but provide less accurate information about the
function $\func$ we wish to optimise.

To provide more intuition for the second condition,
recall that for the SE kernel, $\inffunc(z) \approx \|z-\zhf\|/\hz$ where $\hz$ is the
bandwidth of $\phiz$.
If $\gunc$ is very smooth across $\Zcal$, then the lower fidelities provide more
information about $g(\zhf,\cdot)$.
One should expect a reasonable strategy
to exploit such information effectively as it is cheaper.
Indeed, large $\hz$ reduces the threshold $\gamma(z)$ across the
entire $\Zcal$, causing $\candfidelst$ to be nonempty and \mfgpucbtwos to
consider lower fidelities extensively before proceeding to $\zhf$.
On the other hand, if $\hz$ is small and $\gunc$ is not smooth across $\Zcal$, the
threshold $\gamma(z)$ will be large for all $z$. 
Then $\candfidelst$ vanishes fast and the algorithm will quickly 
skip lower fidelities and proceed to $\zhf$.
%Thus, this behaviour of \mfgpucbtwos is sensible in the SE kernel case. %we are repeating this too often
It is worth noting that the second condition is similar in
spirit to~\citet{kandasamy16mfbo} where they proceed from a lower to higher
fidelity only when the lower fidelity variance is smaller than a threshold.
However, while they treat the threshold as a hyper-parameter, we are able to explicitly
specify theoretically motivated values for it.


Finally, the third condition in~\eqref{eqn:candfidelst},
$\inffunc(z) > \inffunc(\diamz)/\betath$, 
says that we should only pick
fidelities where the information gap $\inffunc$ is large. 
%Since $\inffunc$ is increasing as we move away from
%$\zhf$, it says we will only consider fidelities outside a neighbourhood of $\zhf$.
Recall that if $\candfidelst$ is empty, \boca{} will choose $\zhf$ by default. But, when it is not empty, we want to prevent pathological situations where we get arbitrarily close to
$\zhf$ but not actually query \emph{at} $\zhf$.
%This condition breaks the continuum and forces \bocas to pick $\zhf$ instead of
%querying very close to it.
Observe that since $\betat$ is increasing with $t$, this neighborhood is shrinking with time
and therefore the algorithm will eventually have the opportunity to evaluate fidelities
close to $\zhf$.
Next, we describe our theoretical results.

\input{theory}


% \subsection{Practical Implementation}
% \label{sec:implementation}


% \subsection{Beyond Continuous Fidelity spaces and Domains}
% \label{sec:extensions}

\textbf{Extensions:}
While we have focused on continuous $\Zcal$ due to their wide ranging
practical applications, many of the ideas here can be extended to other settings.
If $\Zcal$ is a discrete subset of $[0,1]^p$ our ideas here can be extended
straightforwardly.
We reiterate that this will \emph{not} be the same as the finite fidelity
\mfgpucbones algorithm  since the assumptions are significantly different.
In particular,~\citet{kandasamy16mfbo} are not able to effectively share
information across fidelities as we do.
We also believe that Algorithm~\ref{alg:mfgpucbtwo} can be extended to arbitrary fidelity
spaces $\Zcal$ as long as a kernel can be defined over $\Zcal$.
% Another avenue for future work would be to study different choices for
% $\Zcal$ kernel where 
% These questions are left for future work.
% In particular when $\Xcal$ is a discrete set, the analysis can be extended in a
% straightforward way.
Our results can also be straightforwardly extended for discrete domains $\Xcal$
and various kernel choices for $\phix$ by mimicking the proofs
from~\citet{srinivas10gpbandits}.
As with most nonparametric methods, \mfgpucbtwos scales poorly with
dimension due to the dependence on $\IGn$.
Due to this reason, we also confine our experiments to small $p,d$.
This can be alleviated by assuming additional structure on
$\func,\gunc$~\citep{djolonga13highdimbandits,kandasamy15addBO}.



